The NuSTAR View of Perseus: the ICM and a Peculiar Hard Excess

As the brightest galaxy cluster in the X-ray sky, Perseus is an excellent target for studying the Intracluster Medium (ICM), but until recently, its active galactic nucleus (AGN) made studies of the diffuse emission near its center nearly impossible to accomplish with NuSTAR due to the extended wings of NuSTAR's PSF. The development of a new open source software package -- nucrossarf -- now allows the contribution from point and diffuse sources to be modeled so that scattered light from the AGN can be accounted for. Using this technique, we present an analysis of diffuse hard X-ray (3-25keV) emission from the ICM using three archival NuSTAR observations of the Perseus cluster. We find a ~10% excess of emission beyond 20keV not describable by purely thermal models. By performing similar analyses of AGN in archival observations, we have characterized the systematic uncertainty of the modeled AGN contribution to be 3.4%. However, in order to explain the excess, the total scattered AGN emission would have to be 39% stronger than we have measured. We test physical explanations for the excess, such as diffuse inverse Compton emission potentially originating from the radio mini-halo, but we determine that none of the models are compelling. An upper limit on inverse Compton flux ($\leq1.5\times10^{-11}$erg s$^{-1}$cm$^{-2}$) and a corresponding lower limit on global magnetic field strength ($\geq 0.35~\mu G$) is derived. We discuss the potential origin and implications of the excess and present our characterization of the nucrossarf systematic uncertainty, which should be useful for future work.

==> Extras/bgd_table.tex <==
\begin{table}[h!]
    \centering
   % \begin{minipage}{0.95\textwidth}
    \begin{center}
    \caption{Best Fit Model Parameters\label{tbl-absorbers}}
    
    
    \begin{tabular}{lllr}
        \\
        \textbf{Model} &  &  &  & \textbf{C-Statistic} \\\addlinespace[0.5ex] \toprule
        \textbf{1T} & & & & \\
        \\
        Apec & T (keV) & 4.47 $\pm$ 0.028 & 5799.93/5605** \\
         & Z (Z_$\odot$) & 0.372 $\pm$ 5.8$\cdot 10^{-3}$  & \\
         %& $z$ & 0.0179 & Fixed & \\
         & Norm & 0.317 & \\ \\\addlinespace[0.5ex]
       
        \midrule
        \textbf{1T + IC} & & & & \\
        \\
        Apec & T (keV) & 4.35 $\pm$ 0.034 & 5767.77/5605 \\
         & Z (Z_$\odot$) & 0.383 $\pm$ 0.00572 & \\
         %& $z$ & 0.0179 & Fixed & \\
         & Norm & 0.311  & \\ 
         \\
         Powerlaw & $\Gamma$ & 2.2 & \\
         & Norm & 4.44 $\cdot$ $10^{-3}$  & \\
        \\
        
        \midrule
        \textbf{2T} & & & & \\
        \\
        Apec$_1$ & T (keV) & 4 $\pm$ 1.0 & 5780.63/5605 \\
         & Z (Z_$\odot$) & 0.3  & \\
         %& $z$ & 0.0179 & Fixed & \\
         & Norm & 1.0e-3  & \\ 
         \\
         Apec$_2$ & T (keV)\footnote[*]{*Actual best fit temperature is ~63**, upper limit was placed at 12 keV} & 4  $\pm$ 1.0 & \\
         %& Z (Z_$\odot$) & 0.3 & Linked to Apec$_1$ & \\
         %& $z$ & 0.0179 & Fixed & \\
         & Norm & 1.0e-3 & \\ 
        \\
        
        %\midrule
        %\textbf{1T * Gaussian} & & & & \\
        %\\
        %Apec & T (keV) & 4 & $\pm$ 1.0 & 1000.0 \\
        % & $Z$ & 0.3 & 1.0 & \\
        % & $z$ & 0.0179 & Fixed & \\
        % & Norm & 1.0e-3 & 1.0 & \\ 
        % \\
        % Gaussian & $\mu$ & 1.7 & $\pm$ 1.0 & 1000.0 \\
        % & $\sigma$ & 0.3 & 1.0 & \\
        % & Norm & 0.3 & 1.0 & \\
        %\\
        	
    \end{tabular}
    \end{center}
    %\vspace{}
   % \end{minipage}
\end{table}




\begin{table*}[h!]
    \caption{Normalization values for background parameters\label{tbl-absorbers}}
    
    \begin{tabular}{ll cccc | cccc}
          & & \multicolumn{4}{c}{\textbf{FPMA}} & \multicolumn{4}{c}{\textbf{FPMB}} 
        \\
         & & 1 & 2 & 3 & 4 & 1 & 2 & 3 & 4 \\
        \toprule
        \multicolumn{10}{c}{\textbf{Observation 90202046002}} \\
        \addlinespace[0.5ex]
        \\
        \textbf{Apeture background} &  & 1.00e+00 & - & - & - & 1.00e+00 & - & - & -
\\
\textbf{CXB} &  & 1.72e-04 & - & - & - & 1.44e-04 & - & - & -
\\
\textbf{Solar Component} & \textbf{Line Energy} & &  &  &  &  &  &  & 
\\
 & 3.54 & 1.03e-02 & 1.09e-02 & 1.55e-02 & 1.08e-02 & 2.83e-02 & 2.78e-02 & 2.52e-02 & 3.90e-02
\\
 & 4.51 & 1.16e-02 & 9.88e-03 & 2.76e-02 & 2.11e-02 & 4.56e-02 & 3.27e-02 & 2.34e-02 & 4.76e-02
\\
 & 10.2 & 1.38e-04 & 2.73e-17 & 1.70e-03 & 2.16e-03 & 1.65e-07 & 1.04e-07 & 7.92e-08 & 1.88e-07
\\
 & 19.65 & 4.51e-04 & 8.78e-05 & 3.36e-04 & 6.53e-04 & 3.66e-04 & 3.41e-04 & 8.90e-04 & 5.91e-04
\\
 & 21.89 & 8.14e-04 & 6.28e-04 & 1.11e-03 & 1.93e-03 & 8.40e-04 & 1.22e-03 & 1.55e-03 & 1.09e-03
\\
 & 22.97 & 2.68e-04 & 2.13e-04 & 2.45e-04 & 3.18e-04 & 2.09e-04 & 2.07e-04 & 2.83e-04 & 2.11e-04
\\
 & 24.75 & 2.87e-03 & 2.33e-03 & 3.84e-03 & 5.01e-03 & 3.50e-03 & 3.85e-03 & 4.50e-03 & 3.68e-03
\\
 & 25.3 & 1.69e-03 & 1.37e-03 & 1.24e-03 & 1.06e-03 & 6.02e-04 & 5.91e-04 & 6.73e-04 & 5.45e-04
\\
 & 27.75 & 1.32e-11 & 1.11e-11 & 6.58e-29 & 1.19e-27 & 7.07e-04 & 7.69e-04 & 8.07e-04 & 7.66e-04
\\
 & 28.08 & 1.10e-16 & 3.23e-15 & 4.83e-03 & 4.63e-03 & 6.12e-11 & 6.12e-11 & 6.12e-11 & 6.12e-11
\\
 & 28.55 & 1.82e-03 & 1.98e-03 & 1.24e-03 & 1.34e-03 & 3.87e-03 & 3.65e-03 & 3.56e-03 & 3.48e-03
\\
 & 30.17 & 7.94e-04 & 6.53e-04 & 1.01e-03 & 1.13e-03 & 9.85e-04 & 8.86e-04 & 1.12e-03 & 1.04e-03
\\
 & 30.86 & 5.28e-03 & 5.26e-03 & 4.54e-03 & 4.26e-03 & 3.57e-03 & 3.73e-03 & 3.67e-03 & 3.43e-03
\\
 & 32.19 & 1.20e-03 & 1.02e-03 & 1.32e-03 & 1.55e-03 & 1.84e-03 & 1.73e-03 & 1.68e-03 & 1.65e-03
\\
 & 35.03 & 4.42e-04 & 4.92e-04 & 4.92e-04 & 3.51e-04 & 3.31e-04 & 3.18e-04 & 2.84e-04 & 3.17e-04
\\
 & 39.25 & 6.08e-03 & 3.84e-03 & 7.63e-03 & 7.98e-03 & 1.29e-02 & 1.20e-02 & 1.30e-02 & 1.33e-02
\\
 & 39.4 & 5.69e-04 & 5.29e-04 & 5.76e-04 & 7.88e-04 & 3.22e-20 & 3.41e-20 & 3.85e-20 & 3.81e-20
\\
 & 47.56 & 2.94e-03 & 2.16e-03 & 3.21e-03 & 2.92e-03 & 3.51e-03 & 3.59e-03 & 3.50e-03 & 3.64e-03
\\
 & 52.5 & 2.27e-03 & 1.83e-03 & 2.45e-03 & 2.89e-03 & 1.56e-03 & 1.64e-03 & 1.78e-03 & 1.72e-03
\\
 & 57.99 & 1.20e-03 & 8.21e-04 & 1.30e-03 & 1.75e-03 & 2.66e-03 & 2.74e-03 & 2.50e-03 & 2.85e-03
\\
 & 65.01 & 4.31e-03 & 3.04e-03 & 5.06e-03 & 6.35e-03 & 3.02e-03 & 2.89e-03 & 3.58e-03 & 3.74e-03
\\
 & 67.06 & 1.58e-20 & 1.89e-20 & 1.30e-20 & 2.00e-20 & 1.46e-03 & 1.40e-03 & 1.10e-03 & 1.28e-03
\\
 & 75.18 & 8.35e-04 & 1.23e-03 & 7.83e-04 & 1.25e-03 & 2.61e-07 & 2.20e-07 & 2.79e-07 & 3.16e-07
\\
 & 85.82 & 5.32e-03 & 5.75e-03 & 6.66e-03 & 6.59e-03 & 5.65e-03 & 4.97e-03 & 5.35e-03 & 4.65e-03
\\
 & 87.9 & 5.21e-03 & 4.87e-03 & 3.48e-03 & 3.89e-03 & 3.68e-03 & 3.97e-03 & 3.63e-03 & 3.97e-03
\\
 & 92.67 & 1.72e-03 & 1.73e-03 & 1.29e-03 & 1.40e-03 & 1.44e-11 & 1.53e-11 & 1.47e-11 & 1.51e-11
\\
 & 105.36 & 1.38e-03 & 1.69e-03 & 8.69e-04 & 1.12e-03 & 5.86e-04 & 6.06e-04 & 5.88e-04 & 6.89e-04
\\
 & 122.74 & 6.86e-13 & 1.14e-12 & 1.89e-13 & 4.78e-13 & 1.84e-21 & 2.36e-21 & 2.38e-21 & 2.46e-21
\\
 & 144.56 & 8.57e-04 & 8.41e-04 & 5.53e-04 & 6.08e-04 & 2.03e-03 & 2.08e-03 & 1.83e-03 & 2.07e-03
\\
\textbf{Low-Energy APEC} &  & 4.01e+00 & 3.41e+00 & 3.90e+00 & 6.72e+00 & 4.29e+00 & 4.03e+00 & 3.00e+00 & 4.06e+00
\\
\textbf{Instrumental Continuum} &  & 5.93e-04 & 6.26e-04 & 6.05e-04 & 6.61e-04 & 6.13e-04 & 5.87e-04 & 6.07e-04 & 6.03e-04
\\
        
        \\
        \\
        
        \midrule
        \multicolumn{10}{c}{\textbf{Observation 90202046004}} \\
        \addlinespace[0.5ex]
        \\
        
        \textbf{Apeture background} &  & 9.95e-01 & - & - & - & 1.00e+00 & - & - & -
\\
\textbf{CXB} &  & 1.72e-04 & - & - & - & 1.74e-04 & - & - & -
\\
\textbf{Solar Component} & \textbf{Line Energy} & &  &  &  &  &  &  & 
\\
 & 3.54 & 1.82e-02 & 1.91e-02 & 2.73e-02 & 1.91e-02 & 1.30e-03 & 1.28e-03 & 1.16e-03 & 1.79e-03
\\
 & 4.51 & 1.44e-02 & 1.23e-02 & 3.43e-02 & 2.63e-02 & 4.42e-02 & 3.17e-02 & 2.27e-02 & 4.61e-02
\\
 & 10.2 & 1.73e-08 & 3.41e-21 & 2.13e-07 & 2.70e-07 & 9.78e-04 & 6.18e-04 & 4.69e-04 & 1.11e-03
\\
 & 19.65 & 2.03e-04 & 3.95e-05 & 1.51e-04 & 2.94e-04 & 8.90e-05 & 8.31e-05 & 2.17e-04 & 1.44e-04
\\
 & 21.89 & 8.83e-04 & 6.82e-04 & 1.21e-03 & 2.09e-03 & 9.06e-04 & 1.31e-03 & 1.67e-03 & 1.17e-03
\\
 & 22.97 & 1.28e-03 & 1.02e-03 & 1.17e-03 & 1.52e-03 & 7.10e-04 & 7.04e-04 & 9.63e-04 & 7.16e-04
\\
 & 24.75 & 2.57e-03 & 2.08e-03 & 3.44e-03 & 4.49e-03 & 2.81e-03 & 3.10e-03 & 3.62e-03 & 2.96e-03
\\
 & 25.3 & 1.66e-03 & 1.35e-03 & 1.22e-03 & 1.04e-03 & 1.03e-03 & 1.01e-03 & 1.15e-03 & 9.33e-04
\\
 & 27.75 & 2.42e-03 & 2.04e-03 & 1.20e-20 & 2.18e-19 & 3.35e-03 & 3.64e-03 & 3.82e-03 & 3.62e-03
\\
 & 28.08 & 1.35e-16 & 3.97e-15 & 5.94e-03 & 5.70e-03 & 2.32e-20 & 2.32e-20 & 2.32e-20 & 2.32e-20
\\
 & 28.55 & 2.56e-03 & 2.78e-03 & 1.75e-03 & 1.89e-03 & 1.99e-03 & 1.88e-03 & 1.83e-03 & 1.79e-03
\\
 & 30.17 & 9.58e-05 & 7.88e-05 & 1.22e-04 & 1.36e-04 & 2.54e-03 & 2.28e-03 & 2.88e-03 & 2.67e-03
\\
 & 30.86 & 5.59e-03 & 5.57e-03 & 4.80e-03 & 4.50e-03 & 4.05e-03 & 4.23e-03 & 4.16e-03 & 3.89e-03
\\
 & 32.19 & 2.71e-04 & 2.30e-04 & 2.96e-04 & 3.48e-04 & 1.77e-03 & 1.66e-03 & 1.62e-03 & 1.58e-03
\\
 & 35.03 & 3.10e-04 & 3.45e-04 & 3.44e-04 & 2.46e-04 & 1.32e-21 & 1.27e-21 & 1.13e-21 & 1.26e-21
\\
 & 39.25 & 8.55e-03 & 5.40e-03 & 1.07e-02 & 1.12e-02 & 8.11e-03 & 7.55e-03 & 8.13e-03 & 8.37e-03
\\
 & 39.4 & 1.04e-03 & 9.64e-04 & 1.05e-03 & 1.44e-03 & 1.22e-03 & 1.30e-03 & 1.46e-03 & 1.45e-03
\\
 & 47.56 & 1.17e-03 & 8.65e-04 & 1.28e-03 & 1.17e-03 & 4.82e-03 & 4.94e-03 & 4.80e-03 & 5.01e-03
\\
 & 52.5 & 1.52e-03 & 1.22e-03 & 1.64e-03 & 1.93e-03 & 1.53e-03 & 1.61e-03 & 1.76e-03 & 1.69e-03
\\
 & 57.99 & 5.18e-03 & 3.54e-03 & 5.62e-03 & 7.54e-03 & 1.67e-03 & 1.72e-03 & 1.57e-03 & 1.79e-03
\\
 & 65.01 & 3.55e-03 & 2.51e-03 & 4.17e-03 & 5.24e-03 & 2.21e-03 & 2.11e-03 & 2.62e-03 & 2.73e-03
\\
 & 67.06 & 1.01e-03 & 1.22e-03 & 8.39e-04 & 1.29e-03 & 1.98e-03 & 1.90e-03 & 1.50e-03 & 1.74e-03
\\
 & 75.18 & 2.77e-03 & 4.07e-03 & 2.59e-03 & 4.13e-03 & 3.77e-03 & 3.18e-03 & 4.02e-03 & 4.56e-03
\\
 & 85.82 & 6.00e-03 & 6.48e-03 & 7.52e-03 & 7.44e-03 & 6.51e-03 & 5.73e-03 & 6.17e-03 & 5.36e-03
\\
 & 87.9 & 3.91e-03 & 3.66e-03 & 2.61e-03 & 2.92e-03 & 2.55e-03 & 2.75e-03 & 2.52e-03 & 2.75e-03
\\
 & 92.67 & 1.41e-03 & 1.42e-03 & 1.06e-03 & 1.15e-03 & 1.15e-03 & 1.22e-03 & 1.18e-03 & 1.21e-03
\\
 & 105.36 & 5.10e-04 & 6.27e-04 & 3.22e-04 & 4.13e-04 & 1.40e-21 & 1.45e-21 & 1.40e-21 & 1.64e-21
\\
 & 122.74 & 4.53e-03 & 7.54e-03 & 1.25e-03 & 3.15e-03 & 2.84e-04 & 3.64e-04 & 3.67e-04 & 3.79e-04
\\
 & 144.56 & 3.28e-03 & 3.22e-03 & 2.12e-03 & 2.33e-03 & 4.98e-03 & 5.12e-03 & 4.50e-03 & 5.09e-03
\\
\textbf{Low-Energy APEC} &  & 2.28e+00 & 1.94e+00 & 2.22e+00 & 3.83e+00 & 4.43e+00 & 4.16e+00 & 3.10e+00 & 4.19e+00
\\
\textbf{Instrumental Continuum} &  & 4.83e-04 & 5.09e-04 & 4.92e-04 & 5.38e-04 & 5.53e-04 & 5.30e-04 & 5.47e-04 & 5.43e-04
\\
        
        \\
        
    \end{tabular}
\end{table*}
\begin{table*}[h!]
    \caption{Norms for Background parameters (continued)\label{tbl-absorbers}}
    
    \begin{tabular}{ll cccc | cccc}
          & & \multicolumn{4}{c}{\textbf{FPMA}} & \multicolumn{4}{c}{\textbf{FPMB}} 
        \\
         & & 1 & 2 & 3 & 4 & 1 & 2 & 3 & 4 \\
        \toprule
        \multicolumn{10}{c}{\textbf{Observation 60061361002}} \\
        \\
        
        \textbf{Apeture background} &  & 1.31e+00 & - & - & - & 7.74e-01 & - & - & -
\\
\textbf{CXB} &  & 1.72e-04 & - & - & - & 1.67e-04 & - & - & -
\\
\textbf{Solar Lines} & \textbf{Line Energy} & &  &  &  &  &  &  & 
\\
 & 3.54 & 4.77e-21 & 5.01e-21 & 7.16e-21 & 5.01e-21 & 1.72e-18 & 1.69e-18 & 1.53e-18 & 2.37e-18
\\
 & 4.51 & 3.10e-20 & 2.64e-20 & 7.36e-20 & 5.64e-20 & 4.65e-22 & 3.34e-22 & 2.39e-22 & 4.85e-22
\\
 & 10.2 & 6.56e-23 & 1.30e-35 & 8.09e-22 & 1.03e-21 & 1.26e-21 & 7.96e-22 & 6.05e-22 & 1.43e-21
\\
 & 19.65 & 6.02e-05 & 1.17e-05 & 4.48e-05 & 8.71e-05 & 3.43e-04 & 3.20e-04 & 8.35e-04 & 5.54e-04
\\
 & 21.89 & 7.11e-04 & 5.49e-04 & 9.71e-04 & 1.68e-03 & 4.82e-04 & 6.99e-04 & 8.90e-04 & 6.24e-04
\\
 & 22.97 & 7.21e-04 & 5.73e-04 & 6.59e-04 & 8.56e-04 & 7.17e-21 & 7.11e-21 & 9.71e-21 & 7.22e-21
\\
 & 24.75 & 1.77e-03 & 1.44e-03 & 2.38e-03 & 3.10e-03 & 3.20e-03 & 3.53e-03 & 4.12e-03 & 3.38e-03
\\
 & 25.3 & 2.28e-03 & 1.84e-03 & 1.67e-03 & 1.43e-03 & 1.81e-03 & 1.78e-03 & 2.03e-03 & 1.64e-03
\\
 & 27.75 & 3.85e-03 & 3.24e-03 & 1.91e-20 & 3.46e-19 & 1.42e-06 & 1.55e-06 & 1.62e-06 & 1.54e-06
\\
 & 28.08 & 1.46e-16 & 4.27e-15 & 6.39e-03 & 6.12e-03 & 2.48e-03 & 2.48e-03 & 2.48e-03 & 2.48e-03
\\
 & 28.55 & 2.89e-03 & 3.14e-03 & 1.98e-03 & 2.13e-03 & 3.53e-03 & 3.33e-03 & 3.24e-03 & 3.17e-03
\\
 & 30.17 & 1.57e-03 & 1.29e-03 & 2.00e-03 & 2.24e-03 & 1.02e-03 & 9.17e-04 & 1.16e-03 & 1.07e-03
\\
 & 30.86 & 3.04e-03 & 3.03e-03 & 2.61e-03 & 2.45e-03 & 4.20e-03 & 4.39e-03 & 4.31e-03 & 4.03e-03
\\
 & 32.19 & 1.00e-03 & 8.52e-04 & 1.10e-03 & 1.29e-03 & 1.00e-03 & 9.39e-04 & 9.14e-04 & 8.95e-04
\\
 & 35.03 & 7.89e-04 & 8.77e-04 & 8.77e-04 & 6.27e-04 & 5.50e-04 & 5.28e-04 & 4.70e-04 & 5.26e-04
\\
 & 39.25 & 6.98e-03 & 4.41e-03 & 8.76e-03 & 9.17e-03 & 9.58e-03 & 8.92e-03 & 9.60e-03 & 9.88e-03
\\
 & 39.4 & 4.69e-04 & 4.35e-04 & 4.74e-04 & 6.49e-04 & 1.80e-04 & 1.91e-04 & 2.15e-04 & 2.13e-04
\\
 & 47.56 & 3.11e-03 & 2.29e-03 & 3.40e-03 & 3.10e-03 & 3.57e-03 & 3.66e-03 & 3.56e-03 & 3.71e-03
\\
 & 52.5 & 2.55e-03 & 2.05e-03 & 2.75e-03 & 3.25e-03 & 1.33e-03 & 1.39e-03 & 1.52e-03 & 1.46e-03
\\
 & 57.99 & 1.95e-03 & 1.33e-03 & 2.11e-03 & 2.83e-03 & 1.60e-03 & 1.65e-03 & 1.51e-03 & 1.72e-03
\\
 & 65.01 & 3.64e-03 & 2.57e-03 & 4.27e-03 & 5.36e-03 & 3.28e-03 & 3.14e-03 & 3.89e-03 & 4.06e-03
\\
 & 67.06 & 2.30e-04 & 2.76e-04 & 1.90e-04 & 2.92e-04 & 3.58e-04 & 3.43e-04 & 2.70e-04 & 3.14e-04
\\
 & 75.18 & 2.47e-03 & 3.63e-03 & 2.31e-03 & 3.68e-03 & 4.27e-03 & 3.60e-03 & 4.56e-03 & 5.17e-03
\\
 & 85.82 & 5.82e-03 & 6.28e-03 & 7.29e-03 & 7.21e-03 & 2.15e-03 & 1.89e-03 & 2.04e-03 & 1.77e-03
\\
 & 87.9 & 4.38e-03 & 4.09e-03 & 2.92e-03 & 3.27e-03 & 5.77e-03 & 6.23e-03 & 5.70e-03 & 6.23e-03
\\
 & 92.67 & 2.21e-03 & 2.23e-03 & 1.66e-03 & 1.80e-03 & 2.36e-03 & 2.51e-03 & 2.41e-03 & 2.47e-03
\\
 & 105.36 & 6.49e-04 & 7.99e-04 & 4.10e-04 & 5.27e-04 & 8.58e-04 & 8.87e-04 & 8.59e-04 & 1.01e-03
\\
 & 122.74 & 1.75e-03 & 2.91e-03 & 4.81e-04 & 1.22e-03 & 6.71e-04 & 8.60e-04 & 8.68e-04 & 8.96e-04
\\
 & 144.56 & 4.41e-03 & 4.33e-03 & 2.85e-03 & 3.13e-03 & 5.50e-03 & 5.66e-03 & 4.97e-03 & 5.62e-03
\\
\textbf{Low-Energy APEC} &  & 1.11e+00 & 9.46e-01 & 1.08e+00 & 1.87e+00 & 9.91e-01 & 9.32e-01 & 6.94e-01 & 9.38e-01
\\
\textbf{Instrumental Continuum} &  & 5.30e-04 & 5.60e-04 & 5.41e-04 & 5.91e-04 & 5.46e-04 & 5.23e-04 & 5.40e-04 & 5.37e-04
\\
        
        
    \end{tabular}
    %\vspace{}
\end{table*}
